Dynamic Correlation Clustering in Sublinear Update Time

We study the classic problem of correlation clustering in dynamic node streams. In this setting, nodes are either added or randomly deleted over time, and each node pair is connected by a positive or negative edge. The objective is to continuously find a partition which minimizes the sum of positive edges crossing clusters and negative edges within clusters. We present an algorithm that maintains an $O(1)$-approximation with $O$(polylog $n$) amortized update time. Prior to our work, Behnezhad, Charikar, Ma, and L. Tan achieved a $5$-approximation with $O(1)$ expected update time in edge streams which translates in node streams to an $O(D)$-update time where $D$ is the maximum possible degree. Finally we complement our theoretical analysis with experiments on real world data.

==> AlgorithmDescription.tex <==
\section{Our Dynamic algorithm}\label{sec: our dynamic algorithm}
\todo[inline]{Algorithm description should be approximately 2 pages}

In this section we describe how to dynamize the static algorithm from \cref{sec:static-algorithm}. In its description we say that two nodes $u$ and $v$ are in agreement if \probabilisticagreement{u}{v}{\epsilon} procedure says so, we also say that a node $u$ is heavy if \heavyprocedure{u}{\epsilon}{\beta} says so. 
%We continue with a high level description of the algorithms before delving into the pseudo-code.
At a very high level, our algorithm tries to mimic the clustering produced by~\cref{alg:vanilla-agreement} in a dynamic way. That is, at each point in time we maintain a sparse solution graph $\Tilde{G_t}$ whose connected components induce a clustering solution for the graph $G_t$.
To form $\Tilde{G_t}$ we dynamically maintain what we call an anchor set, that is a set of nodes such that all edges of $\Tilde{G_t}$ have at least one endpoint which is in the anchor set. These nodes should be thought as representatives of a dense substructure in our graph, which we wish to discover.
A central sub-procedure in our algorithm, which permit us to keep track of evolving clusters is the Notify procedure.
We believe that the latter procedure may be of independent interest and we devote~\cref{subsec: notify procedure} to its description.


\subsection{Notify procedure}\label{subsec: notify procedure}
We design a message-passing procedure, which we call $\mathrm{Notify}$, to communicate events across neighboring nodes. Roughly, this procedure propagates information about the arrival or deletion of a node $u$ to a $O(\polylog n)$-size randomly chosen subset of nodes within small hop distance from $u$. We distinguish between different types of notifications depending on how many nodes did the notification propagate through from the ``source'' node that initiated the notify procedure.

Notifications are subdivided in categories depending on their type, which could be $\T{i}, i = 0,1,2$.
A central definition in our algorithm and in its analysis is the ``interesting event'' definition.

\begin{definition}
   We say that $u$ participates in an ``interesting event'' either when $u$ arrives or $u$ receives a $\T{0}$ or $\T{1}$ notification.
\end{definition}


% \nnote{given that we use I for interesting events, maybe we should call this set $F_u$}
To simplify the description of the algorithm. We denote by $d(u)$ the current degree of a node $u$ and we define the function $l(x) = \floor{\log (x)}, \forall x > 0$. With a slight abuse of notation for a node $u$ we denote by $l_u$ the quantity $l(d(u))$. Note that for all nodes $u$ we have that $2^{l_u} \leq d(u) < 2^{l_u+1} $.

Each node $u$ stores sets $I^0_u, I^1_u,  I^2_u, \dots, I^{\log n}_u$ and $B^0_u, B^1_u,  B^2_u, \dots, B^{\log n}_u$. Set $I^i_u$ contains $u$'s last neighborhood sample when its degree was in $[2^i, 2^{i+1})$ and set $B^i_u$ contains all nodes $v$ such that $u \in I^i_v$. 

Each time a node $u$ participates in an ``interesting event'' or receives a $\T{2}$ notification it stores a random sample of size $O (\log n)$ of its neighborhood in $I^{l_u}_u$. At the same time, $u$ enters the sets $B^{l_u}_v$ for all nodes $v \in I^{l_u}_u$ that it just sampled. Those nodes are responsible to notify $u$ when they get deleted. Thus, upon $u$'s deletion all nodes in $\bigcup_{i} B^i_u$ are notified.

The high level properties regarding when a node $u$ gets notified are: (1) $u$ gets notified and participates in an ``interesting event'' when a constant fraction of its neighborhood gets deleted; and (2) $u$ gets notified when its $2$-hop neighborhood changes substantially.
All these while maintaining the expected complexity bounded by $O(\polylog n)$ each time the \emph{Notify} procedure is called.

\cref{algo:notify} contains the pseudocode of the notification procedure.

\begin{algorithm}
\label{algo:notify}
\caption{Notify($ u, \epsilon$)}
\label{algo:notify}
\begin{algorithmic}
\IF{$u$ arrived}
    \STATE $I^{l_u}_u \xleftarrow{} $  sample $10^{100} \log n / \epsilon$ random neighbors
    \STATE $\forall v \in I^{l_u}_u$: $B^{l_u}_v \xleftarrow{} B^{l_u}_v \cup \{ u\}$
    \STATE $\forall v \in I^{l_u}_u$: $u$ sends $v$ a $\T{0}$ notification
\ELSIF{$u$ was deleted}
    \STATE $\forall v \in \bigcup_i B^i_u$: $u$ sends $v$ a $\T{0}$ notification
\ENDIF
\FOR{$i = 0, 1, 2$}
    \FORALL{$w$ that received a $\T{i}$ notification}
        \STATE $\forall v \in I^{l_w}_w$: $B^{l_w}_v \xleftarrow{} B^{l_w}_v \setminus \{ w\}$
        \STATE $I^{l_w}_u \xleftarrow{} $  sample $10^{100} \log n / \epsilon$ random neighbors
        \STATE $\forall v \in I^{l_w}_w$: $B^{l_w}_v \xleftarrow{} B^{l_w}_v \cup \{ w\}$
        \IF{$i \in \{0, 1\}$}
            \STATE $\forall v \in I^{l_w}_w$: $w$ sends $v$ a $\T{i+1}$ notification
        \ENDIF
    \ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

\newcommand{\np}[1]{%
  \if\relax#1%
    \mathrm{Notify}(\cdot)(\epsilon)% No argument provided, show "Type"
  \else% Argument provided, show "Type_i"
    \mathrm{Notify}({#1})(\epsilon)%
  \fi}

When a vertex $u$ is inserted it first sample $\frac{10^{100}\log n}{\epsilon}$ many of its neighbors, for each such neighbor $v$ vertex $u$ enters $B_{v}^{l_u}$, and sends a $\T{0}$ notification to $v$.
Instead, when a vertex $u$ is deleted it simply sends a a $\T{0}$ notification to every vertex $v\in \bigcup_i B^i_u$.
All vertices $u$ receiving a $\T{i}$ notification, for $i=0,1,2$, $u$ is removed from all sets $B^{l_u}_v$ where  $v\in \I^{l_u}_u$, then it resamples set $\I^{l_u}_u$ and enters $B_{v}^{l_u}$ for all $v$ in the freshly sampled $\I^{l_u}_u$.
The $\T{i}$ notifications, for $i=1,2$, are propagated via the sets $\I^{l_u}_u$ of the vertices $u$ that received $\T{i}$ notifications, for $i=0,1$, respectively.

When a node is added, at most $\polylog n$ notifications are sent, resulting in time complexity $O(\polylog n)$. However this is not given when a node is deleted. Indeed, the deletion of a vertex $u$ results in $O(|\bigcup_i B^i_u| \cdot \polylog n)$ notifications sent in total. 


\subsection{Our Dynamic algorithm pseudocode}
Our~\cref{alg:dynamicagreement} contains 4 procedures: the $\text{Notify}(v_t, \epsilon)$ procedure which we described in~\cref{subsec: notify procedure}, the Clean($ u, \epsilon, t$) procedure, the Anchor($ u, \epsilon, t$) procedure and the Connect($ u, \epsilon, t$) procedure. Before describing the last three we introduce some auxiliary notation. 

We denote by $\I_t$ the set of nodes that participated in an ``interesting event'' at round $t$.
We also denote by $\Phi$ a dynamically changing (across the execution of our algorithm) subset of the nodes which we call anchor set. We avoid the subscript $t$ in the set $\Phi$ notation as it is always clear for the context at what time we are referring to. When a vertex $u$ is deleted, then, we also apply $\Phi \gets \Phi \setminus \{u\}$. We maintain a sparse graph $\Tilde{G_t}$ with the same node set of $G_t$ and with edge set $\Tilde{E_t} \subseteq E_t$. We start our algorithm with $\Tilde{G_0}$ being an empty graph. The backbone of our sparse solution $\Tilde{G_t}$ is the anchor set nodes $\Phi$. Indeed, we have that $\forall e = (u, v) \in \Tilde{E_t}$ either $u$ or $v$ are in $\Phi$. Moreover, for any node $u$ we denote by $\Phi_u$ the subset of the nodes of $\Phi$ with which it is connected in our sparse solution $\Tilde{G_t}$.


\renewcommand{\algorithmicwhile}{\textbf{on arrival/deletion of}}
\renewcommand{\algorithmicendwhile}{\algorithmicend\ \textbf{on}}

\newcommand{\LFORALL}[1]{\State\algorithmicforall\ #1\ \algorithmicdo}
\newcommand{\ELFORALL}{\unskip\ \algorithmicend\ \algorithmicforall}

\begin{algorithm}
\caption{Dynamic Correlation Clustering (DCC)}\label{alg:dynamicagreement}
\begin{algorithmic}
%\STATE {\bfseries Initialization:} $ \xleftarrow{} \emptyset$
\WHILE{$v_t$}
    \STATE $\text{Notify}(v_t, \epsilon)$
    \FORALL{$u \in \I_t$}
        \STATE Clean($ u, \epsilon, t$)
        \STATE Anchor($ u, \epsilon, t$)
        \STATE Connect($ u, \epsilon, t$)
    \ENDFOR
\ENDWHILE
\end{algorithmic}
\end{algorithm}


After the arrival or deletion of node $v_t$ and the propagation of notifications through the $\text{Notify}(v_t, \epsilon)$ procedure, for all nodes $u$ that participated in an important event we do the following: 
\begin{enumerate}
    \item First we call the Clean($ u, \epsilon, t$) procedure which is responsible to delete edges between nodes which are not in $\epsilon$-agreement anymore and delete from the anchor set nodes that lost too many edges in our sparse solution from the time they entered $\Phi$. These operations enable our algorithm to ``destroy'' clusters which are becoming sparse or the nodes in them are not anymore in $\epsilon$-agreement.
    \item Secondly we check if $u$ is heavy. If it is then we flip a coin and with probability $\min \{ 1, \nicefrac{10^{50}\log n}{\epsilon |N_{G_t} (u)|} \}$ we add this node to $\Phi$. If $u$ is added in $\Phi$ then we calculate  agreements with all of its neighbors and whenever $u$ is in agreement with a neighbor $v$ we add edge $(u, v)$ to our sparse solution $\Tilde{G_t}$.
    \item Finally, we initiate the \textit{Connect} procedure. In the latter procedure, $u$ samples approximately $\nicefrac{10^{50}\log n}{\epsilon}$ 
    %\nnote{should be consistent with the constant in the pseudo-code, Fixed} 
    of its neighbors. Let $v$ be one of those sampled neighbors. Then for all $w \in \Phi_v$, if $w$ and $u$ are in agreement then we add the edge $(u, w)$ to $\Tilde{G_t}$.
\end{enumerate}

\begin{algorithm}
\caption{Connect($ u, \epsilon, t$)}\label{alg:connect}
\begin{algorithmic}
\STATE Let $J_u$ be a random sample of size $\nicefrac{10^{50} \log n}{\epsilon}$.
\FOR{$w \in J_u$}
    \FOR{$r \in \Phi_w$}
        \STATE If $r$ is heavy and in agreement with $u$ then add the edge $(r, w)$ to $\Tilde{G_t}$
    \ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Anchor($ u, \epsilon, t$)}\label{alg:anchor}
\begin{algorithmic}
%%%%%%%%%%%%%%%%%%%%
\STATE $X_u \sim \text{Bernoulli}(\min \{ \nicefrac{10^{50} \log n}{\epsilon|N_{G_t}(u)|}, 1\})$
 \IF{$u \in \Phi$}
        \STATE Delete all edges $(u, v)$ where $v \not \in \Phi$ from the sparse solution
    \ENDIF
    \IF{$u$ is heavy and $X_u = 1$}
        \STATE For every neighbor $v$, if $u$ and $v$ are in agreement add edge $(u, v)$ in our sparse solution $\Tilde{G_t}$.
    \ENDIF
    \IF{$X_u = 1$}
        \STATE Add $u$ to $\Phi$ at the end of iteration $t$
    \ELSIF{$ u \in \Phi$ and $X_u = 0$}
        \STATE Delete $u$ from $\Phi$ at the end of iteration $t$
    \ENDIF
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Clean($ u, \epsilon, t$)}\label{alg:clean}
\begin{algorithmic}
%%%%%%%%%%%%%%%%%%%%
\FOR{$w \in \Phi_u$}
    \IF{$w$ not in agreement with $u$ or $w$ is not heavy}
        \STATE Delete edge $(w, u)$ from $\Tilde{G_t}$
    \ENDIF
    \IF{$w$ lost more than an $\epsilon$ fraction of its edges in $\Tilde{G_t}$ from when it entered $\Phi$}
        \STATE Delete $w$ from $\Phi$ and all edges between $w$ and its neighbors in $\Tilde{G_t}$
    \ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> ModelAndPreliminaries.tex <==
\section{Model and preliminaries}
We introduce the \textit{Database model} where the graph $G = (V, E)$ is stored in a database and we can get information regarding the graph through the following queries:
\begin{itemize}
    \item Does edge $(u, v)$ exists?
    \item What is the degree of node $u$.
    \item For every node $u$ we can sample uniformly at random one of its neighbors.
    \item For every node $u$ we can get its entire neighborhood $N(u)$.
\end{itemize}
We naturally assume that the first three queries cost us $\Theta (1)$ and that the last query costs $\Theta (N(u))$. We will argue at the end that all these operations can be (easily) implemented in the classical computational model and only get a poly-logarithmic overhead.


\paragraph{Main goal:} We want to have a dynamic algorithm which maintains a constant factor approximation clustering in:
\begin{itemize}
    \item total update time $O ( n \polylog n) $
    \item expected update time per node insertion to be $O ( \polylog n ) $.
\end{itemize}


==> NewAllfoundsclustersaredense.tex <==
\newcommand{\ta}[1]{t_{#1}^{\text{arrival}} }
\newcommand{\tl}[1]{t_{#1}^{\text{last}} } % version 1
\newcommand{\Canchor}{C_{\Phi}}
\newcommand{\Cnotanchor}{C_{\overline{\Phi}}}
\newcommand{\Nt}[2]{N_{\widetilde{G}_{#1}}(#2) } % version 1


\section{New all found clusters are dense.}\label{sec: New all found clusters are dense}

\begin{definition}\label{def: Mv and Av}
For a node $v \in C$ and t  we define the following events:
\begin{align*}
    T_i^{v, t} &= \left\{  v \text{ received a } Type_i \text{ notification at time } t \right\}\\
    T_i^{v, t, t'} &= \left\{  v \text{ received a } Type_i \text{ notification during the interval } (t, t'] \right\}\\
    \mathcal{T}^{v, t, t'} &= \left\{  v \text{ participated in an ``interesting event'' during the interval } (t, t'] \right\}\\
    A_v^{t} &= \left\{ \left\{ v \in \I_{t}\right\} \lor \left\{ v \text{ received a } Type_2 \text{ notification at time } t\right\} \right\}\\
    M_v^{t, t'} &= \{|\N{t}{v} \setminus \N{t'}{v}| \leq \nicefrac{\epsilon}{10^{5}}|\N{t}{v}| \}\\
\end{align*}
\end{definition}

\begin{lem}\label{lem: When my degree drops I get notified}
Let $u \in V$ and times $t', t $ where $t < t'$. Then:
\begin{equation*}
    \prob \left[  A_v^t \land \overline{T_0^{v, t, t'}} \land \overline{M_v^{t, t'}} \right] < 1/n^{10^{4}}
\end{equation*}
\end{lem}


\begin{definition}
    For every node $v \in V$ and times $t, t'$ where $t < t'$ and a positive integer $d$:
    \begin{align*}
       P_{d, t, t'}^v =  \left( \N{t'}{v} \setminus \N{t}{v}\right) \cap  \left\{ w: \exists t'' \in (t, t']:  |\N{t''}{w}| < 10^{2}d \right\}\
    \end{align*}
\end{definition}

\begin{lem}\label{lem: bound on Adu}
 For every node $v \in V$, time $t'$ and a positive integer $d$:
    \begin{align*}
    \prob [ \left\{|P_{d, t_v, t'}^v| > \epsilon/10^{2} d \right\}] < 3 / n^{10^{3}}
    \end{align*}
\end{lem}


\newcounter{importantdefinitioncounter}
\setcounter{importantdefinitioncounter}{\value{definition}}
\begin{restatable}{definition}{defeventnotmanylosesnotmanynewnodes}\label{def:event such after tu, nodes neither lose too many neighbors nor they get new neighbors of low degree}
\begin{align*}
    \mathcal{R} = 
        &\bigcap_{u \in C, t>t_u } M_u^{t_u, t}
        \bigcap_{u \in C, d\in \left[1, n \right]}
            \left\{
                |P_{d, t_v, \tc}^v| \leq \epsilon/10^{2} d 
            \right\}
\end{align*}
\end{restatable}{definition}
From~\cref{lem: When my degree drops I get notified},~\cref{lem: bound on Adu}, and using the union bound we get the following:
\begin{obs}\label{obs: R happens with high probability}
\begin{align*}
\prob \left[ \mathcal{R} \right] > 1 - 1/n^{10^{2}}    
\end{align*}
\end{obs}
In addition, by the definition of event $\mathcal{R}$:
\begin{obs}\label{obs: Ntu can only increase with high degree nodes}
    $\mathcal{R}$ implies that for all $v \in C$ and $ t \in (t_v, \tc]$:
    \begin{enumerate}
    \item  $|\N{t_v}{v} \setminus \N{t}{v} | \leq \epsilon/{10^{5}} |\N{t_v}{v} |$; and
    \item  $|\left( \N{t}{v} \setminus \N{t_v}{v}\right) \cap  \left\{ u : |\N{t}{u}| < 10^{2} |\N{t}{v}| \right\}| \leq \epsilon / 10^{2} |\N{t}{v}|$
\end{enumerate}
\end{obs}


\begin{lem}\label{lem: anchor set nodes do not change their neighborhood too much}
    Let $u \in \C$ and $t > t_u$ a time when $u$ is in $\epsilon$-agreement with $v$, and either $u$ or $v$ is $\epsilon$-heavy. Then $\mathcal{R}$ implies that:
    $$
    (1 + 10 \epsilon) |\N{t_u}{u}| \geq |\N{t}{u}| \geq (1 - \epsilon/10^{5}) |\N{t_u}{u}|
    $$
\end{lem}



\begin{cor}\label{cor: anchor set nodes do not change their neighborhood too much}
   Let $u \in \C$ and $t \geq t_u$ a time when $u$ is in $\epsilon$-agreement with $v$, and either $u$ or $v$ is $\epsilon$-heavy. Then $\mathcal{R}$ implies that:
    \begin{enumerate}[ref=(\arabic*) of Corollary \thecor]
        \item  $|\N{t_u}{u} \setminus \N{t}{u}| \leq \epsilon/10^{5} |\N{t_u}{u}| <  \epsilon / 10^{4}  |\N{t}{u}|$; and \label{cor: Nt remains the same p1}
        \item $|\N{t}{u} \setminus \N{t_u}{u}| \leq 6 \epsilon |\N{t}{u}| < 7 \epsilon  |\N{t_u}{u}|$\label{cor: Nt remains the same p2}
    \end{enumerate}
\end{cor}


\begin{lem}\label{lem: anchor set nodes do not change their neighborhood too much properties}
    Let $u \in \Canchor$ and $t > t_u$. Then $\mathcal{R}$ implies that:
    \begin{enumerate}[ref=(\arabic*) of Lemma \thelem]
        \item $\Nt{t_u}{u} \subseteq \N{t_u}{u}$\label{lem: Nttu is stable p1}
        \item $|\N{t_u}{u} \setminus \Nt{t_u}{u}| < \epsilon |\N{t_u}{u}|$\label{lem: Nttu is stable p2}
        \item $|\Nt{t_u}{u}| \geq (1 - \epsilon) |\N{t_u}{u}|$\label{lem: Nttu is stable p3}
        \item $|\Nt{t_u}{u} \setminus \Nt{t}{u}| < \epsilon |\Nt{t_u}{u}|$\label{lem: Nttu is stable p4}
        \item $|\Nt{t}{u} \setminus \Nt{t_u}{u}| < 8 \epsilon |\N{t_u}{u}|$\label{lem: Nttu is stable p5}
        \item $|\Nt{t}{u} \setminus \Nt{t_u}{u}| < 12 \epsilon |\Nt{t_u}{u}|$\label{lem: Nttu is stable p6}
        \item $|\Nt{t}{u} | < (1 + 12 \epsilon) |\Nt{t_u}{u}|$\label{lem: Nttu is stable p7}
        \item $( 1 - \epsilon) |\Nt{t_u}{u} | < |\Nt{t}{u}|$\label{lem: Nttu is stable p8}
    \end{enumerate}
\end{lem}


\begin{ineq}\label{ineq: set inequality}
     Let $A, B, C$ and $D$ be four sets, then:
     \begin{align*}
             |A \cap B| \geq |C \cap D| - |C \setminus A| - |D \setminus B|
     \end{align*}
 \end{ineq}


\begin{lem}\label{lem: anchor set nodes have a high overlap if the interesection is nonempty}
    Let $u, v \in \Canchor$ and $t' \geq \max \{ t_u, t_v\}$  such that $\Nt{t'}{u} \cap \Nt{t'}{v}$ is non-empty. Then $\mathcal{R}$ implies that: $|\Nt{t'}{u} \cap \Nt{t'}{v}| \geq (1 -  80 \epsilon)  \max \{ |\Nt{t'}{u}|, |\Nt{t'}{v}| \}$. 
\end{lem}


% Old lemmas instead of having tcurrent they have t larger than in max {t_u, t_v } in their statement.
\begin{lem}\label{lem: two anchor sets have a non empty intersection in our sparse solution}
    $\mathcal{R}$ implies that $\forall u, v \in \Canchor$: $\Nt{\tc}{u} \cap \Nt{\tc}{v} \neq \emptyset$.
\end{lem}


\begin{cor}\label{cor: main corolarry lower bounding the interesection of the neighborhoods between two anchor set nodes in the sparse solution}
    Let $u, v \in \Canchor$, $\mathcal{R}$ implies that $|\Nt{\tc}{u} \cap \Nt{\tc}{v}| \geq (1 -  80 \epsilon)  \max \{ |\Nt{\tc}{u}|, |\Nt{\tc}{v}| \}$.
\end{cor}

\begin{obs}\label{lem: min implies max implies min set inequalities}
     For sets $A, B$, $C$ and positive reals $\alpha, \beta$: 
    \begin{enumerate}
    \item If $|A \triangle B| \leq \epsilon \max \{|A|, |B| \}$ then $|A \cap B| \geq (1 - \epsilon) \max \{|A|, |B| \}$.
    \item If $|A \cap B| \geq (1 - \epsilon) \max \{|A|, |B| \}$ then for $\epsilon$ small enough:\\
    $$|A \triangle B| \leq 2 \epsilon \max \{|A|, |B| \} \leq \frac{2 \epsilon}{1 - \epsilon} \min \{|A|, |B| \} \leq 3 \epsilon \min \{|A|, |B| \}$$
    \item If $|A \triangle B| \leq \epsilon \max \{|A|, |B| \}$ then for $\epsilon$ small enough $|A \triangle B| \leq 3 \epsilon \min \{|A|, |B| \}$
    \item $|A \triangle C| \leq |A \triangle B| + |B \triangle C|$.
    \item $\alpha \min \{|A|, |B| \} + \beta \min \{|B|, |C| \} \leq (\alpha + \beta ) \max \{ |A|, |C|\}$
\end{enumerate}
\end{obs}


\newcommand{\Nh}[2]{N_{\widehat{G}_{#1}}(#2) } % version 1

\begin{thm}\label{thm: C is dense}
$\mathcal{R}$ implies that cluster $C$ is dense and $\forall v \in C$:
    $$
    |\N{\tc}{v} \cap C| \geq (1 - 541080 \epsilon) |C|
    $$
    and 
    $$
    |\N{t_u}{v}| \geq  | C| /2.
    $$
\end{thm}

==> NewDenseClustersFinding.tex <==
\section{New finding dense clusters}\label{sec: New finding dense clusters}

\begin{obs}\label{obs: bounds on degree of u at time tc wrt C}
$\forall u \in C$ we have:
$$
(1 - \epsilon/10^{13}) |C| \leq |\N{\tc}{u}| \leq (1 + \epsilon/10^{13}) |C|
$$
\end{obs}

\begin{obs}\label{obs: at tc u is connected to almost everybody in C}
$\forall u \in C$ we have:
$$
|\N{\tc}{u} \cap C| \geq (1 - \epsilon/10^{13}) |C|
$$
\end{obs}

\begin{obs}\label{obs: at time t the v is connected with most nodes in C}
For each $u\in C$ that arrived at time $t \in [t',\tc]$ we have:
$$
|\N{t}{u} | \geq |\N{t}{u} \cap C | \geq (1 - 2 \epsilon/ 10^{4})|C|
$$
\end{obs}

\begin{obs}\label{obs: C minus Ni is upper bounded}
For each $u\in C$ that has already arrived before time $t \in [t',\tc]$ we have:
$$
|C \setminus \N{t}{u} | \leq 2 \epsilon/  10^{4}|C| \leq  \epsilon/  10^{3}|\N{t}{u}|
$$
\end{obs}

\begin{definition}\label{def: Mv and Av}
For a node $v \in C$ and time $t$ we define the following events:
\begin{align*}
    M_v^{t} &= \{|\N{t}{v} \setminus \N{\tc}{v}| < \nicefrac{\epsilon}{8 \cdot 10^{4}}|\N{t}{v}| \}\\
    A_v^{t} &= \left\{ \left\{ v \in \I_{t}\right\} \lor \left\{ v \text{ received a } Type_2 \text{ notification at time } t\right\} \right\}
\end{align*}
\end{definition}


\begin{lem}\label{lem: high degree implies very different neighborhood}
    $\forall v \in R \cup L^i$ we have that if $M_v^{t_i}$ is true then:
    \begin{align}
        & |\N{t_i}{v}| < (1 + \nicefrac{\epsilon}{2 \cdot 10^{4}}) |C|\\
        &|\N{t_i}{v} \setminus C| < \nicefrac{\epsilon}{10^{4}} |C| < \nicefrac{\epsilon}{ 10^{3}}|\N{t_i}{v}|
    \end{align}
\end{lem}

\begin{lem}\label{lem: Oui and Ow suffice for ui and w being in agreement}
For all neighboring nodes $ v, u \in R \cup L^i$: if $M_v^{t_i} \land M_u^{t_i}$ is true then $v$ and $u$ are in $\epsilon/10$-agreement.
\end{lem}

\begin{lem}\label{lem: different neighborhood has very low probability}
    $\forall v \in C$ and time $t$ we have that:
    $$
    \prob[\overline{M_v^{t}} \land A_v^{t} \land \{ v \in R \cup L^i\} \land \{t \geq t_i \}] < 1/n^{10^{4}}
    $$
\end{lem}

\begin{definition}\label{def: random set D_{t_i}}
    For $t_i$ we define the random set: $ D_{t_i} = \{  v : v\in \N{t_i}{u_i} \cap (R \cup L^i)  \land \overline{M_v^{t_i}} \}$.
\end{definition}


\begin{lem}\label{lem: almost all nodes have almost their final neighborhood at time ti}
    $\forall t_i$ we have that:
    $$
    \prob[ |D_{t_i}| \geq \epsilon/10^{5}  |\N{t_i}{u_i}|] < 1/n^{10^{3}}
    $$
\end{lem}


\begin{thm}\label{thm: ui are heavy}
    If $ \{ |D_{t_i}| < \epsilon/10^{5}  |\N{t_i}{u_i}| \} \land M_{u_i}^{t_i}$ is true then $u_i$ is $\epsilon/10$-heavy at time $t_i$. In addition, if $u_i$ also enters the anchor set at time $t_i$ then it remains in it at least until time $\tc$.
\end{thm}

\begin{definition}\label{def: random set Tv}
    For $v \in C$ we define the random set:
    $$
    T_v = \left\{i \in \{1,2,\dots, \lfloor \epsilon/10^{4} |C| \rfloor \}: \overline{M_v^{t_i}} \land \{ (u_i, v) \in E_{t_i} \} \right\}
    $$
\end{definition}


\begin{lem}\label{lem: v in R has almost the same neighborhood as its final neighborhood for the largest part of the last important events}
Let $v \in R \cup L_1$, then
$$
\prob [|T_v| \geq \epsilon/10^{5} |C| ] < 1 / n^{10^{2}}
$$
\end{lem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{lem}\label{lem: all nodes in R get selected by some node in A1}
For every node $v \in R$ let 
\begin{align*}
    X_v = \left\{ \exists i \in [\epsilon/(2\cdot 10^{4}) |C| ]: 
\{u_i \in L_1 \text{ enters the anchor set }\} \land \{ (v, u_i) \in  E_{t_{i'}}, \forall i' \in [i, \tc] \right\}
\end{align*}
then $\prob [X_v] > 1 - 1/n^{10} $.
\end{lem}

\begin{lem}\label{lem: all nodes in L1 get selected by some node in L2}
For every node $v \in L_1$ let 
\begin{align*}
    X_v = \left\{ \exists i \in \{\epsilon/(2\cdot 10^{4}) |C| + 1,  \dots, \epsilon/10^{4} |C|\} ]: 
\{u_i \in L_2 \text{ enters the anchor set }\} \land \{ (v, u_i) \in  E_{t_{i'}}, \forall i' \in [i, \tc] \right\}
\end{align*}
then $\prob [X_v] > 1 - 1/n^{10} $.
\end{lem}


\begin{lem}\label{lem: all nodes in L2 get connected trough the Connect procedure}
    For every node $u_j \in L_2$ let 
    \begin{align*}
    X_{u_j} = \left\{ \exists i \in [\epsilon/(2\cdot 10^{4}) |C| ]: 
\{u_i \in L_1 \text{ enters the anchor set }\} \land \{ (u_j, u_i) \in  E_{t_{i'}}, \forall i' \in [t_j, \tc] \right\}
\end{align*}
then 
\begin{align*}
    \prob [ X_{u_j} ] \geq 1 - 1/n^{10}
\end{align*}
\end{lem}

\begin{thm}\label{thm: all nodes of C are clustered together}
   With probability at least $(1 - 1/n^{8})$ all nodes of $C$ are clustered together at time $\tc$ by our algorithm.
\end{thm}
